Analysis of Bayesian Networks via Prob-Solvable Loops

Prob-solvable loops are probabilistic programs with polynomial assignments over random variables and parametrised distributions, for which the full automation of moment-based invariant generation is decidable. In this paper we extend Prob-solvable loops with new features essential for encoding Bayesian networks (BNs). We show that various BNs, such as discrete, Gaussian, conditional linear Gaussian and dynamic BNs, can be naturally encoded as Prob-solvable loops. Thanks to these encodings, we can automatically solve several BN related problems, including exact inference, sensitivity analysis, filtering and computing the expected number of rejecting samples in sampling-based procedures. We evaluate our work on a number of BN benchmarks, using automated invariant generation within Prob-solvable loop analysis.

==> notes.tex <==
%!TEX root = main.tex



\section*{Notes and Thoughts - On the links between BNs and PPs, in particular \ProbModel{}}

\subsection*{PPs analysis}

When it comes to (automatic) PP analysis, especialy loop analysis, there is an obvious trade-off between the complexity of the class of programs to be analysed (complexity of the language used) and the amount of information we can capture (usefulness loop invariant).

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.45\linewidth]{fig/tradeoff}
%	%\caption{} 
%	\label{fig:tradeoff}
%\end{figure}


\subsection*{BNs}

BNs give us a succint way of representing complex distributions. If we can encode BN in \ProbModel{}, we can use them to draw values for program variables from these distributions. On the other hand, we can use PPs, and \ProbModel in particular, as a tool to work with BNs. There's a lot of work on analysing BNs, e.g. exact and approximate inference, or sensitivity analysis. In some cases, this can be done within the \ProbModel{} setting.


\subsection*{Two approaches to PP analysis}

\begin{enumerate}
	\item as probabilistic systems over state-space given by the program variables
	\item as deterministic systems over state-space of probability distributions
\end{enumerate}


Let's have a closer look at the second approach. 
Space of distributions may be (and in general is) too complex and complicated to deal with. On the other hand, the reasoning and computations become deterministic.

We can make the distribution-space simpler by projecting it down, i.e. represent the distributions with EV only. Or with moments as in \ProbModel{}. Or with MGFs, CFs, BNs, ... Different projections capture different properties and can be applied to different program classes.

\begin{remark} Projection to expected values, as often done in PP analysis, is inadequate not only because the information we retain is limited, but in some cases it's not sufficient to do the reasoning at all. Consider a simple update $x:=\Normal(0,1); y:=y+x^2$. 
If the projection simplifies the space to just EVs of program variables, i.e. $E[x]$ and $E[y]$, the update of $y$ is characterized by $E[y] \to E[y] + E[x^2]$, so $E[y]$ directly depends on the second moment of $x$. The projection to EVs simplifies the problem too much.
\end{remark}

%Each program update is just a shift in the distribution-space, determined by the current position and the update itself. 

We have to find the delicate balance between projection that simplify too much, hence making it impossible to reason about the program, and simplifying too little, and making it impossible to reasonably represent and interpret the results.

\begin{remark} In \ProbModel{} and \Mora{} the projection is set automatically to the right moments to be able to compute MBIs specified by goal.
\end{remark}


\subsection*{Back to BNs}

One way to represent complex probability/distribution space in a concise way is through BNs (that's exactly what they're for). Maybe we can represent the program with a sequence of (finite) BNs. With each update (or loop iteration) specifying a transition to the new BN. Guards (in loops and if-else) are essentially inferences. What updates give BN-transitions that can be represented reasonably, dealt with? What projection would simplify sufficiently but not overly?


\begin{itemize}
	\item [$\to$] We can work with BNs and (some) inference in \ProbModel{} (PPs).
	\item [$\to$] We can work with \ProbModel{} (PPs) as BNs.
\end{itemize}


\subsection*{Projections, Complexity-Information Tradeoff}

(table)

\begin{table}[h]
\centering
\begin{adjustbox}{width=1.5\textwidth,center=\textwidth}
\begin{tabular}{lllll}
	\hline
	Invariants/Method 	&  Problem addressed	 &  Class & Projection & Ref.		\\
	\hline \hline
	BNs			 		& 	$\forall?$	& (very simple)		& BNs &		\\
	CFs			 		& 	$\forall?$	& (very simple)		& CFs & 		\\
	Moments, MBIs 	&  loop invariant generation	 &   \ProbModel{}  & Moments & 	\citep{probsolvable, mora}\\
	Martingales: template-based (deg), poly. (if $\exists$) 	&  termination,  &  PTS & EVs of bded deg polys & 	\citep{schreuder2019} using SOS	\\
	--- 	&  ERT	 &  BNL & --- & \citep{howlong}		\\
	Martingales: EVs of lin. combinations 	&  termination, 	 &  --- & EVs of program variables		\\
	\hline
\end{tabular}
\end{adjustbox}
\caption{The table shows some methods used for analysing PPs. ordered (roughly) by how much information is captured}
\end{table}

% AST
% PAST
% AS persistence
% AS recurrence
% ERT
% sensitivity
% differential properties
% (bi)simulation/equivalence
% 


% martingales - from transitions rather than overall loop behaviour. what property (lin/poly over prog vars) is (semi-)preserved across transitions? somewhat like looking at local structure and using that for overall behaviour



